Combining Machine Learning and Sampling-Based Search for Multi-Goal Motion Planning with Dynamics

This paper considers multi-goal motion planning in unstructured, obstacle-rich environments where a robot is required to reach multiple regions while avoiding collisions. The planned motions must also satisfy the differential constraints imposed by the robot dynamics. To find solutions efficiently, this paper leverages machine learning, Traveling Salesman Problem (TSP), and sampling-based motion planning. The approach expands a motion tree by adding collision-free and dynamically-feasible trajectories as branches. A TSP solver is used to compute a tour for each node to determine the order in which to reach the remaining goals by utilizing a cost matrix. An important aspect of the approach is that it leverages machine learning to construct the cost matrix by combining runtime and distance predictions to single-goal motion-planning problems. During the motion-tree expansion, priority is given to nodes associated with low-cost tours. Experiments with a vehicle model operating in obstacle-rich environments demonstrate the computational efficiency and scalability of the approach.

==> Sections/bigtable.tex <==
\begin{table*}[htbp]
% \vspace{-10mm}
    \renewcommand\arraystretch{1.3}
    \small
  \centering
  \setlength\tabcolsep{5pt}
  \caption{If it failed to find a solution, the distance is 3000 and duration is 2000}
  \label{tab:freq}
  \begin{tabular}{|p{4em}|p{7em}|p{3em}p{3em}p{3em}p{3em}|p{3em}p{3em}p{3em}p{3em}|}
    \hline
    Scene & Planner 
    & \multicolumn{4}{c|}{Distance (mean)}
    & \multicolumn{4}{c|}{Duration (mean)} \\
    \cline{3-10}
     &  & 20 &  30 & 40 & 50 & 20 &  30 & 40 & 50 
    \\ 
    \hline
 & Lu & 562.2 & 726.2 & 873.6 & 1008.3 & 331.7 & 425.1 & 519.2 & 589.7\\
& 0T + 1D & 551.9& 736.2& 876.3& 1008.6& 326.5& 432.7& 511.8 & 594.6\\
Random & 1T + 0D & 636.7 &838.3 &1010.4 & 1154.4& 365.0& 483.5& 579.9 &668.6\\
(Scene 1)& 0.2T + 0.8D &574.3 &735.9 &895.2 &1022.6 &338.2 &432.3 & 524.4 & 604.7\\
& DROMOS & 411.3&522.3 &614.5 & 690.9& 237.8 & 304.1& 361.6 & 413.0\\
& DROMOS-Rand &1020.6 & 1483.4 & 1838.6& 2194.2 &642.9 & 924.9 & 1136.6 & 1325.5 \\
\hline
 & Lu & 712.2 & 906.2 & 1064.4 & 1235.0 & 418.7 & 527.5 & 623.0 & 721.4\\
& 0T + 1D & 696.0& 886.2& 1070.9&1226.3 & 402.8& 516.8& 624.0 & 712.1\\
Curves & 1T + 0D &809.3 &1023.7 & 1246.4& 1390.6& 461.0& 578.2& 718.0 &787.4\\
(Scene 2)& 0.2T + 0.8D & 705.6& 917.9& 1089.2&1235.4 &412.2 &541.7 &  626.5& 724.9\\
& DROMOS & 495.7&627.0 &727.0 & 818.9&284.2 & 366.4& 424.8 & 482.6\\
& DROMOS-Rand & 1129.1 & 1573.2 & 2114.7 & 2976.6 & 698.0& 964.2 & 1242.3 & 2000+\\
\hline
 & Lu & 784.7&1002.5 & 1181.8&1324.5 & 458.9& 586.5&  692.5& 781.7\\
& 0T + 1D &786.0 & 1008.4&1182.2 &1292.3 &459.6 & 586.3& 697.2 & 758.1\\
Maze & 1T + 0D &903.8 & 1237.8& 1413.1& 1582.9& 526.9& 711.3& 828.5 &929.0\\
(Scene 3)& 0.2T + 0.8D &784.9 & 1009.7&1182.2 & 1325.8&456.2 &586.3 & 703.5 & 779.0\\
& DROMOS & 507.5&626.2&721.4 & 794.5&295.1 &364.3& 421.8 & 467.6\\
& DROMOS-Rand &2231.9 & 2955.0& 3000+ & 3000+ & 2000+ & 2000+ & 2000+ & 2000+\\
\hline
 & Lu &723.1 & 898.2& 1052.0& 1236.8&430.4 &526.7 & 620.6 &725.8 \\
& 0T + 1D & 739.1& 890.2&1044.8 &1234.0 &435.5 &522.3 & 614.1 &729.4 \\
Trap & 1T + 0D &808.9 & 992.7& 1187.5&1382.8 & 462.2&575.2 & 628.4 &798.7\\
(Scene 4)& 0.2T + 0.8D & 706.4& 896.2& 1058.1& 1250.0& 413.7&528.0 & 617.9 & 733.5\\
& DROMOS & 506.20&614.0&703.8 & 778.9&289.6 &357.4& 414.0 & 463.0\\
& DROMOS-Rand & 1219.0 & 2001.1 & 2523.1 & 2991.1 & 746.4 & 1048.1 & 2000+  & 2000+ \\
\hline
\end{tabular}
\end{table*}
